A collaboration to support novice instructors in research-based astronomy teaching

Introductory astronomy is one of the most widely-taken university science courses and a common means of satisfying general education requirements. This course is frequently taught in large sections by a variety of instructors, some with little formal training in astronomy. Thus, instructors often struggle to help students connect with what is typically their last formal science experience. At California State University Fullerton, we have engaged in reform efforts in the teaching of introductory astronomy. We report on the model of reform implementation with several key features that we believe were instrumental in our success. First, our astronomy instructors learned to use research-based curricular materials by attending workshops before and after first implementation. Second, the astronomy instructors collaborated with student Peer Instructors as a team to document and reflect on the implementation progress. Third, the instructional team of faculty and Peer Instructors worked with science education researchers to collect information on common student conceptual difficulties, and develop strategies to address these difficulties using resources in the research and teaching literature. Our findings suggest that this is a fruitful and sustainable model for reform implementation, faculty professional development, and research on the teaching and learning of astronomy.

==> bibitems-old.tex <==
This is the old bibitems before Josh added everything to references.bib

%\begin{thebibliography}{99}
%% The numeral (here 99) in curly braces is nominally the number of entries in
%% the bibliography. It's supposed to affect the amount of space around the
%% numerical labels, so only the number of digits should matter--and even that
%% seems to make no discernible difference.
%
%\bibitem{Hake1998} R. R. Hake, “Interactive-engagement versus traditional methods: A six-thousand-student survey of mechanics test data for introductory physics courses,” \textit{Am. J. Phys.} 66(1), 64–74 (1998).
%
%\bibitem{dber2012}\url{http://www.nap.edu/catalog.php?record_id=13362}
%
%\bibitem{Prather2009} Prather, E.E. , Rudolph, A.L., Brissenden, G., and Schlingman, W.M., A National Study Assessing the Teaching and Learning of Introductory Astronomy. Part I. The Effect of Interactive Instruction. (2009) Am. J. Phys., 77 (4), 320, DOI:10.1119/1.3065023
%
%\bibitem{Rudolph2010} Rudolph, A.L., Prather, E.E. , Brissenden, G., Consiglio, D. and Gonzaga, V., A National Study Assessing the Teaching and Learning of Introductory Astronomy. Part II. The Connection between Student Demographics and Learning. (2010) Astronomy Education Review, 9, 1, DOI:10.3847/AER0009068
%
%\bibitem{Meltzer2012}\url{http://www.per-central.org/items/detail.cfm?ID=12019}
%
%\bibitem{Mazur1997}\url{http://mazur.harvard.edu/education/pi_manual.php}
%
%\bibitem{McDermott2002}McDermoott, L., \& Schaffer, P. (2002). \textit{Tutorials in introductory physics}. Upper Saddle River, NJ: Prentice Hall. 
%
%\bibitem{Prather2004} Research on a Lecture-Tutorial Approach to Teaching Introductory Astronomy for Non–Science Majors, Edward E. Prather, Timothy F. Slater, Jeffrey P. Adams, Janelle M. Bailey, Lauren V. Jones and Jack A. Dostal, \textit{AER} \textbf{3}, 122 (2004); http://dx.doi.org/10.3847/AER2004019
%
%\bibitem{Bardar2006}Development and Validation of the Light and Spectroscopy Concept Inventory, Erin M. Bardar, Edward E. Prather, Kenneth Brecher and Timothy F. Slater, \textit{AER} \textbf{5}, 103 (2006); \url{http://dx.doi.org/10.3847/AER2006020}
%
%\bibitem{Bailey2007}Development of a Concept Inventory to Assess Students’ Understanding and Reasoning Difficulties about the Properties and Formation of Stars
%Janelle M. Bailey, \textit{AER} \textbf{6}, 133 (2007); http://dx.doi.org/10.3847/AER2007028
%
%\bibitem{Henderson2010}Barriers to the use of research-based instructional strategies: The influence of both individual and situational characteristics, \textit{Phys. Rev. ST Phys. Educ. Res.} \textbf{3}, 020102 (2007).
%
%\bibitem{Henderson2009} C. Henderson M. H. Dancy, ``Impact of physics education research on the teaching of introductory quantitative physics in the United States," \textit{Phys. Rev. ST Phys. Educ. Res.} \textbf{5}, 020107 (2009).
%
%\bibitem{Shulman1986}Those Who Understand: Knowledge Growth in Teaching Lee S. Shulman Educational Researcher, Vol. 15, No. 2 (Feb., 1986), pp. 4-14 \url{http://www.jstor.org/stable/1175860}.
%
%\bibitem{Seeds2012}Foundations of Astronomy, Michael Seeds, Dana Backman, 12th edition, Cengage Learning, 2012.
%
%\bibitem{Bennett2012}The Essential Cosmic Perspective with Mastering Astronomy, 6th ed, Bennett, Donahue, Schneider and Voit (Addison-Wesley/Pearson),
%ISBN 0321715365.
%
%\end{thebibliography}
